Idempotent and tropical mathematics and problems of mathematical physics (Volume I)

This volume contains the proceedings of an International Workshop on Idempotent and Tropical Mathematics and Problems of Mathematical Physics, held at the Independent University of Moscow, Russia, on August 25-30, 2007.

==> allauthstring.tex <==
\newpage
\section*{LIST OF PARTICIPANTS AND AUTHORS}
\vskip0.3cm
\label{list-of-pars}
\thispagestyle{empty}
\avtor{AKIAN Marianne}{\INRIA}{France}{\\Marianne.Akian@inria.fr}
\avtor{BAKLOUTI Ali}{Dep\-art\-ment of Math\-ema\-tics,   Fac\-ulty of
 Sci\-en\-ces at Sfax, Rou\-te de Sou\-kra, 3038, Sfax}{Tunisia}{Ali.Baklouti@fss.rnu.tn}
\avtor{BELAVKIN Viacheslav P.}{School of Math\-ema\-ti\-cal Sci\-en\-ces,
Not\-ting\-ham Uni\-ver\-sity, NG7 2RD}{United Kingdom}{Viacheslav\_Belavkin@nottingham.ac.uk} 
\thispagestyle{empty}
\rusavtor{BENIAMINOV Evgeny M.}%
{Бениаминов Евгений Михайлович}{Russian State Uni\-ver\-sity
for the Hum\-ani\-ties, Fac\-ulty of Math\-ema\-tics,
\mbox{ul. Chayanova 15}, Moscow}%
{Russia}{ebeniamin@yandex.ru}
\rusavtor{CHOURKIN Andrey V.}{Чуркин Андрей Валерьевич}%
{\fizfak}{Russia}%
{churandr@mail.ru}
\thispagestyle{empty}
\rusavtor{DANILOV Vladimir I.}{Данилов Владимир Иванович}%
{CEMI RAS, Nahi\-mov\-ski prosp. 47,
117418, Moscow}{Russia}{\\vdanilov43@mail.ru}
\avtor{FARHI Nadir}{\INRIA}{France}{\\Nadir.Farhi@inria.fr}
\thispagestyle{empty}
\avtor{FAYE Farba}{Dep\-art\-ment of Math\-ema\-tics \& Com\-pu\-ter Sci\-ence, UCAD, Dakar}
{Senegal}{\\lamffaye@yahoo.fr}
\rusavtor{FOCK Vladimir V.}{Фок Владимир Владимирович}%
{ITEP, B.~Che\-re\-mush\-kin\-skaya~25, Mos\-cow}{Russia}{fock@itep.ru}
\avtor{GAUBERT St\'ephane}{\INRIA}{France}{\\Stephane.Gaubert@inria.fr}
\rusavtor{GEL'FAND Alexander M.}{Гельфанд Александр Маркович}{\delfin}
{Russia}{\\gelfand\_a@oaoesp.ru}
\avtor{GONCHAROV Alexander B.}%
{Brown Uni\-ver\-sity, Math. Dep\-art\-ment, \mbox{151 Thayer st.}, Pro\-vid\-ence, RI}%
{USA}{Alexander\_Goncharov@brown.edu}%
\thispagestyle{empty}
\rusavtor{GRBI\'C Tatjana}{Грбич Татjана}{\novisadg }{Serbia}%
{tatjana@uns.ns.ac.yu}
\rusavtor{GULINSKY Oleg V.}{Гулинский Олег Викторович}{IPPI RAS,
B.~Ka\-ret\-ny~1, Mos\-cow}{Russia}{bedelbaeva\_aigul@mail.ru}
\avtor{GUREVICH Dmitry}{LAMAV, Uni\-ver\-site de 
Va\-len\-cien\-nes,\\ Le Mont Houy 59313 Va\-len\-cien\-nes}{France}%
{d.gurevich@free.fr}
\thispagestyle{empty}
\rusavtor{GUTERMAN Alexander E.}{Гутерман Александр Эмильевич}%
{\mehmat}{Russia}{guterman@list.ru}
\avtor{IGONIN Sergey}{Utrecht University, NL-3508 TA Utrecht}{\\The Netherlands}{igonin@mccme.ru}
\avtor{ITENBERG Ilia}{\IRMA}{France}{itenberg@math.u-strasbg.fr}
\rusavtor{KARZANOV Alexander V.}{Карзанов Александр Викторович}%
{ISA RAS, prosp. 60-le\-tiya Ok\-tya\-brya 6, 117312, Mos\-cow}{Russia}%
{\\sasha@cs.isa.ru} 
\avtor{KHARLAMOV Vyacheslav}{\IRMA}{France}{kharlam@math.u-strasbg.fr}
\rusavtor{KIRSHTEYN Boris Kh.}{Кирштейн Борис Хаймович}{\delfin}
{Russia}{\\bkirsh@aha.ru}
\thispagestyle{empty}
\rusavtor{KOLOKOLTSOV Vassili N.}{Колокольцов Василий Никитич}%
{Moscow Institute of Eco\-no\-mics, Pe\-cher\-ska\-ya~ul.~6/1, 129344, \mbox{Moscow},
and the Uni\-ver\-sity of War\-wick, Dept. of Sta\-tis\-tics, Cov\-en\-try CV4 7AL}
{Russia and United Kingdom}{vkolok@fsmail.ru}
\thispagestyle{empty}
\rusavtor{KOSHEVOY Gleb A.}{Кошевой Глеб Алексеевич}%
{\CEMI}{Russia}{\\gleb\_koshevoy@mail.ru}
\rusavtor{KOVAL Gennady V.}{Коваль Геннадий Васильевич}%
{\fizfak}{Russia}
{kovgen@mail.ru}
\rusavtor{KUSHNER Alexey G.}{Кушнер Алексей Гурьевич}%
{Astrakhan State University, ul. Tatischeva 20a, 414056, Astrakhan}%
{Russia}{kushnera@mail.ru}
\rusavtor{KUTATELADZE Simon S.}{Кутателадзе Семен Самсонович}%
{S.L.~Sobolev Math\-ema\-ti\-cal Ins\-ti\-tute, prosp. Kop\-tyu\-ga 4, 630090, 
\mbox{Novosibirsk}}{Russia}{sskut@math.nsc.ru}
\thispagestyle{empty}
\rusavtor{LITVINOV Grigory L.}{Литвинов Григорий Лазаревич}
{\nezavisimy}{\\Russia}{glitvinov@gmail.com}
\rusavtor{MASLOV Victor P.}{Маслов Виктор Павлович}%
{\fizfak}{Russia}{v.p.maslov@mail.ru}

\avtor{MCCAFFREY David}
{7th floor, St. James buil\-ding, 79 Ox\-ford Street,
Man\-che\-ster M1 6SS}{United Kingdom}{david@mccaffrey275.fsnet.co.uk}

\avtor{MCENEANEY William M.}{Dept. of Mech\-ani\-cal and 
Aer\-osp\-ace Engi\-nee\-ring, MC 0411,
Uni\-ver\-sity of Cali\-for\-nia, San Diego
9500 Gil\-man Drive,
La Jolla, CA 92093-0411}{USA}{wmceneaney@ucsd.edu}

\rusavtor{MIKHALKIN Evgeny N.}{Михалкин 
Евгений Николаевич}{\krasped}%
{Russia}{mikhalkin@bk.ru}

\rusavtor{MOLCHANOV Vladimir F.}{Молчанов Владимир
Федорович}{\tambov}{Russia}{molchano@molchano.tstu.ru}

\avtor{NITICA Viorel}{\romanian\ and Dept. of Mathematics, West Chester University, PA}{Romania and USA}
{vnitica@wcupa.edu}

\avtor{PAP Endre}{\novisadps}{Serbia}{pap@im.ns.ac.yu}
\thispagestyle{empty}
\avtor{PERSSON Ulf}{Chalmers University of Tech\-no\-logy, 412 96 G\"{o}\-te\-borg}{Sweden}{\\ulfp@math.chalmers.se}
\avtor{QUADRAT Jean-Pierre}{\INRIA}{France}{\\Jean-Pierre.Quadrat@inria.fr}
\rusavtor{RASHKOVSKII Alexander Yu.}
{Рашковский Александр Юрьевич}{University of Sta\-van\-ger,
4036 Sta\-van\-ger}{Norway}
{\\alexander.rashkovskii@uis.no}

\rusavtor{SERGEEV Serge\u{\i} N.}{Сергеев Сергей Николаевич}
{\fizfak}{Russia}
{sergiej@gmail.com}

\rusavtor{SHPIZ Grigory B.}{Шпиз Григорий Борисович}{\nezavisimy}{\\Russia}{shpiz@theory.sinp.msu.su}

\avtor{SHUSTIN Eugenii}{School of Math\-ema\-ti\-cal Sci\-en\-ces, Tel Aviv Uni\-ver\-sity, Ra\-mat Aviv, Tel Aviv,\\ 69978}%
{Israel}{shustin@post.tau.ac.il}
\thispagestyle{empty}

\rusavtor{SHVEDOV Oleg Yu.}{Шведов Олег Юрьевич}
{\fizfak}{Russia}
{olegshv@mail.ru}
\thispagestyle{empty}

\avtor{SINGER Ivan}{\romanian}{Romania}{ivan.singer@imar.ro}

\rusavtor{SOBOLEVSKI\u{I} Andre\u{\i}}{Соболевский Андрей Николаевич}{\fizfak}{Russia}{ansobol@gmail.com}

\rusavtor{STOYANOVSKY Alexander V.}{Стояновский Александр Васильевич}{\nezavisimy}{Russia}{stoyan@mccme.ru}
\thispagestyle{empty}

\rusavtor{\v{S}TRBOJA Mirjana}{Штрбоjа Мирjана}{\novisadps}{Serbia}%
{mirjanas@im.ns.ac.yu}

\avtor{THIAM Mamadou}{\sengalese}{Senegal}{\\mathiam@netcourier.com}
\thispagestyle{empty}
\avtor{TRUFFET Laurent}{Institut de Recherche en Com\-mu\-ni\-ca\-tions et Cy\-ber\-ne\-tique de Nantes,
IRCCyN UMR-CNRS 6597, 1, rue de la Noe BP 92101 44321 Nantes Cedex}{France}
{Laurent.Truffet@emn.fr}


\rusavtor{TSYKINA Svetlana V.}{Цыкина Светлана Викторовна}
{\tambov}{Russia}%
{tsykinasv@yandex.ru}

\rusavtor{ULVERT Roman V.}{Ульверт Роман Викторович}{\krasfed}{Russia}{ulvertrom@yandex.ru}
\thispagestyle{empty}

\avtor{WAGNEUR Edouard}{\'Ecole Polytechnique de Mon\-tr\'e\-al, C.P.~6079 Succ. Cen\-tre-ville,
Mon\-tr\'eal Qu\'e\-bec H3C 3A7, and
GERAD, Montreal}{Canada}{Edouard.Wagneur@gerad.ca}
\thispagestyle{empty}

\avtor{WALSH Cormac}{\INRIA}{France}
{\\cormac.walsh@inria.fr}
\thispagestyle{empty}

\rusavtor{ZNAMENSKAYA Oksana V.}%
{Знаменская Оксана Витальевна}%
{\krasfed}%
{Russia}{znamensk@lan.krasu.ru}

\thispagestyle{empty}
